ORCA: The Annealed Spectral Conditioning Optimizer for Faster, Better LLM Training

Modern LLM optimizers such as Muon often produce weight matrices with higher effective rank than Adam, yet further spectral control has delivered only modest gains. We identify a tension behind this result: concentrated spectra can suppress gradient directions in coupled weight matrices and slow optimization, while constraints maintained throughout training can limit task-specific adaptation and raise the attainable loss floor. We introduce ORCA (Orthogonal Regularization, Cooled After), a minimal optimizer intervention that applies strong but temporary soft orthogonality regularization early in training, then removes it. This allows the weights to benefit from a broader spectrum early on and adapt freely afterward. Across LLaMA, Qwen3, and fine-grained mixture-of-experts models ranging from 130M to 8B parameters, ORCA achieves lower final validation loss than Muon. Its loss reduction relative to Muon matches or exceeds Muon's reduction relative to Adam. Ablations support the early-shaping, later-release design. Further, ORCA requires no architectural changes and adds minimal overhead. An implementation is available at https://github.com/uuurraaa/ORCA_Optimizer.

==> arxiv/sections/section3_final.tex <==
\section{Spectral Structure and Optimization}

As noted in Section 1, Muon’s higher effective rank coincides with faster optimization. This observation suggests that properties of the weight spectrum may be useful for optimization, but whether they provide a general benefit remains unclear. To turn this still-vague possibility into a precise question about optimization dynamics, we ask:
\begin{center}
\fbox{
\parbox{0.92\linewidth}{
\centering
\textbf{Q1.}
\emph{Can the spectral structure observed under Muon directly affect
optimization speed, and through what mechanism?}
}}
\end{center}

A direct mechanism already appears in 'the multiplicatively coupled weight
matrices' of Transformers. Consider for example the value--output pair $\mathbf W_V\mathbf W_O$ of a single attention
head:
\begin{equation}
\operatorname{Attn}(\mathbf H)
=\operatorname{softmax}\!\left(
\frac{\mathbf H\mathbf W_Q\mathbf W_K^\top\mathbf H^\top}{\sqrt{d_h}}
\right)\mathbf H\mathbf W_V\mathbf W_O .
\end{equation}
The gradient of the value projection takes the form
\[
\nabla_{\mathbf W_V}L
=
\mathbf G\mathbf W_O^\top,
\quad \text{with} \quad
\mathbf G=\nabla_{(\mathbf W_V\mathbf W_O)}L .
\]
Here, $\mathbf G$ denotes the gradient with respect to the entire product
$\mathbf W_V\mathbf W_O$.
Thus, $\mathbf W_O$ acts as a spectral filter on the gradient received by
$\mathbf W_V$. Writing
$\mathbf W_O=\sum_i \sigma_i\mathbf u_i\mathbf v_i^\top$, we have
$\nabla_{\mathbf W_V}L
=\sum_i \sigma_i(\mathbf G\mathbf v_i)\mathbf u_i^\top$.
This makes the role of the spectrum explicit: each component
$\mathbf G\mathbf v_i$ enters the gradient with weight $\sigma_i$.
If $\mathbf W_O$ is scaled orthogonal,
$\mathbf G\mathbf W_O^\top$ preserves the spectrum of $\mathbf G$ up to a
common scale. At the opposite extreme, if $\mathbf W_O$ has rank $r$,
the update is restricted to contributions from $r$ spectral directions.
More generally, as the spectrum becomes more concentrated, directions
associated with smaller singular values contribute proportionally less to
the update.

In fact, this partner-dependent filtering is ubiquitous in Transformers:
analogous coupling appears between the query--key pair
$(\mathbf W_Q,\mathbf W_K)$ and the up- and down-projections of MLP and expert
blocks.

To isolate this mechanism from the surrounding Transformer computation, consider the generic factorization $\mathbf W=\mathbf X\mathbf Y$, where $\mathbf G=\nabla_{\mathbf W}L(\mathbf W)$.
The simple chain rule gives
\(
\nabla_{\mathbf X}L
=\mathbf G\mathbf Y^\top,
\nabla_{\mathbf Y}L
=\mathbf X^\top\mathbf G,
\)
so each factor directly filters the gradient received by its partner. Under the
continuous-time exact-polar Muon dynamics \citep{ambrosio2005gradient,peyre2026muon},
\[
\dot{\mathbf X}
=-\eta_t^X\operatorname{Polar}(\mathbf G\mathbf Y^\top),
\qquad
\dot{\mathbf Y}
=-\eta_t^Y\operatorname{Polar}(\mathbf X^\top\mathbf G),
\]
where $\operatorname{Polar}(\mathbf M)=\mathbf U\mathbf V^\top$
for an SVD $\mathbf M=\mathbf U\mathbf\Sigma\mathbf V^\top$.
The instantaneous loss decrease is therefore
\[
-\dot L
=\eta_t^X\Nnorm{\mathbf G\mathbf Y^\top}
+
\eta_t^Y\Nnorm{\mathbf X^\top\mathbf G} .
\]
Thus, the same filtered gradients above are the quantities that determine Muon's instantaneous loss decrease. The local
spectral effect can therefore translate into a local effect on optimization speed.

To empirically demonstrate this effect, we conduct a reciprocal $V$--$O$ intervention.
Let $\mathbf G_O=\nabla_{\mathbf W_O}L$ denote the gradient with respect to
$\mathbf W_O$, and let $\mathbf U_O=\operatorname{Polar}(\mathbf G_O)$ denote
the corresponding Muon update direction.
At a 10k-step checkpoint, we raise the smaller singular values of $\mathbf W_V$
toward its largest singular value while keeping its singular vectors and spectral
norm fixed, and update only $\mathbf W_O$ with Muon.
As shown in \Cref{fig:v-rank-o-metrics}, with the Muon update scale
$\|\mathbf U_O\|_F$ held fixed, increasing the effective rank of $\mathbf W_V$
increases $\|\mathbf G_O\|_*$---the loss decrease under Muon
flow---while decreasing the gradient--weight alignment
$\cos(\mathbf G_O,\mathbf W_O)$.
These all indicate that the same-sized Muon update has a stronger effect as the effective rank of
$\mathbf W_V$ increases.
Consistently, \Cref{fig:v-rank-o-surface} also shows that updating $\mathbf W_O$
yields a larger held-out loss decrease at higher effective rank of $\mathbf W_V$.

\begin{figure}[htb]
  \centering
  \captionsetup{font=small,skip=4pt}
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/singular_blue.png}
    \caption{Absolute singular-value spectra.}
    \label{fig:v-rank-o-spectrum}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/v_rank_o_key_metrics.pdf}
    \caption{Gradient and update metrics.}
    \label{fig:v-rank-o-metrics}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[trim=0 0 0 12,clip,width=\linewidth]{figures/v_rank_o_loss_surface.pdf}
    \caption{Held-out loss decrease.}
    \label{fig:v-rank-o-surface}
  \end{subfigure}
  \captionsetup{skip=2pt}
  \caption{Single-layer $V$-spectrum intervention with $O$-only Muon updates.
  $\mathbf G_O$ and $\mathbf U_O$ denote the gradient and Muon update direction.
  In (c), rollout steps and loss decrease use logarithmic scales.}
  \label{fig:v-rank-o-diagnostics}
\end{figure}

These observations suggest a simple principle: spectral concentration can create an optimization bottleneck. For a nonzero matrix $\mathbf A$, define its effective rank by $\erank(\mathbf A):=\Fnorm{\mathbf A}^2/\Snorm{\mathbf A}^2$.
To make this intuition concrete, we study a matrix-factorization model. The following bounds illustrate one possible mathematical pathway through which spectral structure may affect optimization.
\vspace{-2pt}
\begin{theorembox}
\begin{boxedtheorem}[Low Effective Rank Limits Descent Speed]
\label{thm:mechanistic}
For $k\ge2$, let $\mathbf X$ and $\mathbf Y$ be conformable matrices with
$\mathbf W=\mathbf X\mathbf Y\in\mathbb R^{k\times k}$, and consider the
column-wise softmax loss
\begin{equation}
 L(\mathbf W)
 =\sum_{i=1}^{k}
 \left[
 \log\!\left(\sum_{j=1}^{k}e^{\mathbf W_{ji}}\right)
 -\mathbf W_{c_i i}
 \right],
\quad c_i\in[k], \quad \text{with} \quad \mathbf{W} = \mathbf{X}\mathbf{Y}
\label{eq:objective}
\end{equation}
let $(\mathbf X_t,\mathbf Y_t)_{t\in[0,T]}$ be an absolutely continuous solution
of the exact-polar Muon flow above, with $\eta_0\ge0$ and
\(
0\le\eta_t^X\le\eta_0/\Snorm{\mathbf Y_t},
\qquad
0\le\eta_t^Y\le\eta_0/\Snorm{\mathbf X_t}.
\)
Assume that the factor norms satisfy
\(
\Snorm{\mathbf X_t},\Snorm{\mathbf Y_t}>0
\)
for all $t\in[0,T]$.
Writing $L_t=L(\mathbf X_t\mathbf Y_t)$, we have
\[
L_T
\ge
 L_0\exp\!\left[
-\sqrt{2}\,\eta_0
\int_0^T
\left(
\sqrt{\erank(\mathbf X_s)}
+
\sqrt{\erank(\mathbf Y_s)}
\right)ds
\right].
\]
\end{boxedtheorem}
\end{theorembox}

\begin{wrapfigure}{r}{0.34\linewidth}
  \centering
  \captionsetup{font=footnotesize,skip=3pt}
  \includegraphics[width=\linewidth]{figures/pso_constraint_comparison.png}
  \captionsetup{skip=2pt}
  \caption{Validation loss under persistent spectral constraints.}
  \label{fig:constraint_levels}
\end{wrapfigure}
\vspace{-2pt}
In this factorization model, the bound relates the rate of loss decrease to the effective ranks of the factors. Naturally, broad spectral support may alleviate this bottleneck, as demonstrated by the intervention experiments in \Cref{fig:v-rank-o-diagnostics}. We therefore test whether maintaining such support throughout LLaMA pretraining helps by imposing progressively stronger spectral constraints. However, \Cref{fig:constraint_levels} shows that persistent orthogonal constraints worsen validation loss.
Thus, the path-side advantage identified above does not translate into a benefit
when the same structure is enforced persistently. This leads to our second
question:
\vspace{-2pt}
\begin{center}
\fbox{
\parbox{0.92\linewidth}{
\centering
\textbf{Q2.}
\emph{If broad spectral structure alleviates an optimization bottleneck,
why enforcing it hurts performance?}
}}
\end{center}
\makeatletter
\par
\WFclear
\ifdim\linewidth<\hsize
  \advance\linewidth\WF@adjlw
  \advance\@totalleftmargin-\WF@adjtlm
\fi
\makeatother
\vspace{-3pt}
The key is that a property that is favorable along the optimization trajectory
need not be favorable when imposed as a persistent constraint.
Spectral control does more than influence how an optimizer moves: when enforced
throughout training, it also restricts the spectral structure of the solutions
that the optimizer is allowed to reach.
For example, an orthogonality constraint
\(
\mathbf{W}\mathbf{W}^\top\approx\mathbf{I}
\)
forces the singular values of $\mathbf{W}$ to remain nearly equal.
If the task prefers a more anisotropic or lower-effective-rank solution, such a
constraint can prevent the optimizer from reaching it.

The factorized model above makes this competing effect concrete.
For the same column-wise softmax objective in
Eq.~\eqref{eq:objective},
the following theorem shows that sufficiently high effective rank can itself
impose a nonzero loss floor.

\begin{theorembox}
\begin{boxedtheorem}[High Effective Rank Can Impose a Loss Floor]
\label{thm:endpoint}
Assume $k\ge2$, $\mathbf W\neq0$, and
\(\|\mathbf W\|_2\le B\) for a fixed scale bound $B=O(1)$. Let
\(
K
=
\left|
\{c_i:i\in[k]\}
\right|
\)
denote the number of distinct target indices. Then
\[
L(\mathbf{W})
\ge
C_k(\mathbf{W})\,k
\left(
1-
\sqrt{
\frac{K}{\erank(\mathbf{W})}
}
\right),
\]
where $C_k(\mathbf{W})>0$ is the scale factor determined by $k$ and
$\|\mathbf{W}\|_F/\sqrt{k}$. The rank factor
$1-\sqrt{K/\erank(\mathbf{W})}$ increases with effective rank and becomes
positive when $\erank(\mathbf{W})>K$.
\end{boxedtheorem}
\end{theorembox}

\vspace{-5pt}

Thus, for this objective, sufficiently high effective rank is not merely
unnecessary at the optimum: it can be incompatible with arbitrarily small
loss. In particular, if $\mathbf{X}$ and $\mathbf{Y}$ are $k\times k$ scaled
orthogonal matrices, then
$\erank(\mathbf{X}\mathbf{Y})=k$, and Theorem~\ref{thm:endpoint} gives the
positive endpoint loss floor
\(
C_k(\mathbf{W})\,k
\left(
1-\sqrt{K/k}
\right)
\)
whenever $K<k$.

Together, these results illustrate a tension in the stylized model: broad spectral support can relax a path-side bottleneck, while a persistent spectral constraint can restrict low-loss solutions. We also test whether these intuitions are useful in the empirical training.
The same spectral property can therefore be useful as a transient feature of
the optimization trajectory while being harmful as a persistent constraint on
the final solution.

This distinction helps reconcile the empirical behavior above.
The high effective rank naturally maintained by Muon can support optimization
without prescribing a fixed spectral geometry for the final weights.
By contrast, increasingly restrictive spectral constraints preserve the desired
structure by reducing the freedom of the model to adapt its spectrum as
training proceeds.
The appropriate goal is therefore not to maximize effective rank at every
point in training, but to retain enough spectral support to avoid path-side
bottlenecks while still allowing the spectrum to adapt to the task.


==> arxiv/sections/section4.tex <==
\section{ORCA: A Minimal Shape-then-Release Optimizer}
\label{sec:orca}

The preceding analysis reveals a tension between the trajectory-side benefit
and the endpoint-side cost of spectral control.
Broad spectral support can facilitate optimization along the training
trajectory, while enforcing the same structure persistently may restrict
task-adaptive solutions at the endpoint.
This suggests a temporal design principle: spectral control should shape the
early optimization trajectory, but be released before it restricts task
adaptation.

ORCA (Orthogonal Regularization, Cooled After) is a minimal two-stage
realization of this shape-then-release principle.
During an initial active stage, ORCA applies spectral shaping to steer the
early trajectory away from spectrally concentrated regimes.
After this stage, the shaping term is removed completely and training reverts
to standard Muon.
This separation allows spectral control to influence the optimization path
without prescribing the spectral geometry of the final solution.

\subsection{Algorithm}
\label{sec:orca-algorithm}

\noindent\textbf{A minimal realization: soft orthogonal shaping.}
For this minimal realization, ORCA uses soft orthogonality as its spectral
shaping operator.
Consider a matrix parameter $\mathbf{W} \in \mathbb{R}^{p \times q}$, and assume
$p \leq q$ for notational simplicity.
We define
$
    \mathcal{R}_{\mathrm{orth}}(\mathbf{W})
    =
    1/4\
    \left\|\mathbf{W}\mathbf{W}^\top-I_p\right\|_F^2 ,
    \label{eq:orca-orth-reg}
$
whose gradient is
\begin{equation}
    G_{\mathrm{orth}}(\mathbf{W})
    :=
    \nabla_{\mathbf{W}}\mathcal{R}_{\mathrm{orth}}(\mathbf{W})
    =
    \left(\mathbf{W}\mathbf{W}^\top-I_p\right)W .
    \label{eq:orca-orth-grad}
\end{equation}

Writing a thin singular value decomposition as
$\mathbf{W}=\mathbf{U}\operatorname{diag}(\sigma_1,\ldots,\sigma_p)\mathbf{V}^\top$, we have
\begin{equation}
\begin{aligned}
    \mathcal{R}_{\mathrm{orth}}(\mathbf{W})
    =
    \frac{1}{4}
    \sum_{i=1}^{p}
    \left(\sigma_i^2-1\right)^2, \quad
    \mathbf{G}_{\mathrm{orth}}(\mathbf{W})
    =
    \mathbf{U}\operatorname{diag}
    \left(
        (\sigma_i^2-1)\sigma_i
    \right)_{i=1}^{p}
    \mathbf{V}^\top .
\end{aligned}
\label{eq:orca-orth-svd}
\end{equation}
Thus, a gradient step on $\mathcal{R}_{\mathrm{orth}}$ decreases singular
values above unit scale and increases nonzero singular values below unit scale,
tending to reduce spectral concentration and increase the effective-rank
measure considered in the preceding analysis.
The operator requires neither an explicit SVD nor a projection onto the
Stiefel manifold and can be computed using matrix multiplications alone.

\noindent\textbf{ORCA update.}
Let $\mathbf{U}_t$ denote the standard Muon update direction at step $t$,
$\eta_t$ the learning rate, $\lambda$ the decoupled weight-decay coefficient,
and $\gamma_t$ the spectral-shaping strength.
For each matrix parameter $\mathbf{W}_t$, the ORCA update can be written as
\begin{equation}
    \mathbf{W}_{t+1}
    =
    \mathbf{W}_t
    -
    \eta_t \mathbf{U}_t
    -
    \eta_t\lambda \mathbf{W}_t
    -
    \eta_t\gamma_t \mathbf{G}_{\mathrm{orth}}(\mathbf{W}_t).
    \label{eq:orca-update}
\end{equation}
The weight-decay and spectral-shaping corrections are both evaluated at the
pre-update parameter $\mathbf{W}_t$ \citep{loshchilov2017decoupled}, while $\mathbf{U}_t$ is computed in the same way as in
standard Muon.

Similar to Muon and other matrix-based optimizers, ORCA is applied only to
matrix parameters in the matrix-optimizer group.
Embeddings, the language-model head, and one-dimensional parameters continue
to follow their original AdamW updates.

\noindent\textbf{Release rule.}
The defining feature of ORCA is that spectral shaping is transient rather than
persistent.
Let $T$ denote the total number of training steps and
$\tau\in[0,1]$ the active fraction.
The active window has length $S$, and we use the hard release schedule
\begin{equation}
  \gamma_t =
  \begin{cases}
  \gamma, & t < S, \\
  0,      & t \geq S,
  \end{cases}
  \qquad
  S = \left\lfloor \tau T \right\rfloor.
  \label{eq:orca-gamma-schedule}
\end{equation}
Equation~\eqref{eq:orca-gamma-schedule} makes the two phases explicit.
During the \emph{active stage} ($t<S$), ORCA augments Muon with the
spectral-shaping term in Eq.~\eqref{eq:orca-update}.
During the \emph{released stage} ($t\geq S$), the shaping term vanishes and
the optimizer reverts exactly to the corresponding standard Muon training
rule.

The hard switch is the simplest implementation of the shape-then-release
principle.
The early intervention is used to steer the optimization trajectory away from
spectrally concentrated regimes, rather than to prescribe a persistent
spectral constraint.
Once released, the spectrum is free to adapt to the task objective.
Empirically, we find that part of the higher-effective-rank state induced
during the active stage persists after release, allowing the optimization
benefit to continue without maintaining the orthogonal regularizer.
Unless otherwise specified, we use $\tau=0.25$ throughout the paper;
Section~5 studies sensitivity to the release point.

\noindent\textbf{Beyond soft orthogonality.}
Soft orthogonality defines the default ORCA optimizer, but the underlying
shape-then-release principle is not tied to this particular spectral operator.
In Section~5, we replace soft orthogonal shaping with alternative early
spectral interventions, including Pion-start and DiagSVD variants.
These methods differ in how the spectral state is shaped during the active
stage; once the active window ends, the intervention is removed and all
variants continue with the same released Muon dynamics.
This provides a controlled way to study whether the benefit of early spectral
intervention extends beyond soft orthogonality itself.

\noindent\textbf{Implementation and overhead.}
In the standard setting, ORCA adds two matrix multiplications per weight matrix during shaping without changing the communication complexity; the remaining operations are fused into the optimizer update. Our Muon baseline performs 24 matrix multiplications across eight Newton--Schulz iterations, so shaping increases the multiplication count by \(2/24=8.3\%\). This extra work disappears after release. We batch matrices of identical shapes to reduce kernel launches, use dedicated kernels, and form the Gram matrix along the shorter dimension. On the 8B MoE model, average distributed optimizer update time is \(227.2\,\mathrm{ms}\) for Muon and \(237.4\,\mathrm{ms}\) for ORCA. The \(10.2\,\mathrm{ms}\) difference amounts to approximately \(0.8\%\) of a roughly \(1.3\,\mathrm{s}\) training step. Peak memory is \(101.41\,\mathrm{GB}\) and \(101.66\,\mathrm{GB}\), respectively. Overall, ORCA incurs negligible additional training overhead in this configuration.

\label{sec:implementation-details}


==> arxiv/sections/section5.tex <==
\section{Experiment Validations}
\label{sec:main-results}
In this section, we verify the efficacy of ORCA on three specific issues: (1) Llama pretraining with grid learning rate search and larger scale pretraining. (2) Pretraining task on Qwen3 architecture with the additional QK-norm that may violate the matrix factoring reparameterization. This section focuses on the efficacy of ORCA, and for more robustness test of parameters and controlled interventions on gain of ORCA, readers can refer to Section~\ref{sec:interventions}.

\subsection{Experimental Setup and Tuning Protocol}
\label{sec:setup}

\textbf{Setups.}  We pre-train Llama-series models \cite{touvron2023llama} ranging from 130M to 1.3B parameters on C4 , using 25B to 100B tokens. We also pre-train Qwen3-series models \cite{yang2025qwen3} ranging from 160M to 0.6B parameters on The Pile \citep{gao2020pile}, using  25B to 100B tokens. Finally, we train fine-grained mixture-of-experts models ranging from 0.8B to 8B parameters on OLMo-mix-1124 \citep{olmo20242}, the data mixture including DCLM-Baseline \citep{li2024datacomp} using 25B to 100B tokens.

We first run a learning rate grid-search for Adam, Muon, Pion and ORCA. All trials share the same data, batch size, sequence length, and 50k-step training budget. We use $\mathbf{O}_t = 0.2/\mathrm{Rms}(\mathbf{O}_t)\cdot \mathbf{O}_t$ to rescale the Muon and ORCA update where $\mathbf{O}_t$ is the Newton-Schulz orthogonalization output to align the update with the Adam's \citep{liu2025muon}.
We perform a two-stage coarse-to-fine learning rate grid search. The coarse sweep evaluates $\{5\times10^{-4},10^{-3},2\times10^{-3},5\times10^{-3}\}$. Once the coarse sweep locates a candidate learning rate, we evaluate the neighbors on its both sides to refine the best lr within a smaller local range. The refinement grid consists of $\{6,8\}\times10^{-4}$, $\{1.3,1.6\}\times10^{-3}$,
and $\{3,4\}\times10^{-3}$, which reduces the local spacing between learning rates candidates to about $1.2\times$--$1.5\times$.  All four optimizers use this protocol and the same tuning budget.

The advantage of ORCA holds over a wide range of learning rates: at every learning rate evaluated for both methods, ORCA reaches a lower final validation loss than Muon, and at all evaluated configurations between $10^{-3}$ and $5\times10^{-3}$ it is even better than fully tuned Muon. The independent searches select $1.3\times10^{-3}$, $3\times10^{-3}$, $10^{-3}$, and $2\times10^{-3}$ for Adam, Muon, Pion, and ORCA, with final validation losses of $2.8824$, $2.8460$, $2.9790$, and $2.8106$, respectively; ORCA thus lowers the loss by a further $0.0354$ relative to the best Muon and stays within $0.002$ of its own optimum across $1.6\times10^{-3}$ to $3\times10^{-3}$, showing that the improvement does not rely on a narrow learning-rate choice.

\label{sec:pretraining}

\textbf{LLama Pretraining Tasks.} We compare ORCA against Adam and Muon on LLaMA 350M and 1.3B, training each model for 100B tokens. As shown in \Cref{fig:main-pretraining}, Muon outperforms Adam at both scales, while ORCA further lowers the validation loss. Compared with Muon, ORCA reduces the final loss by $0.0194$ at 350M and $0.0244$ at 1.3B, with consistent gains at both scales. Further, a four-seed robustness result for the 130M, 50k-step setting is reported in
Appendix~\ref{app:more-experiment-results}.
We also evaluate the final ORCA and Muon LLaMA 1.3B checkpoints from \Cref{fig:main-pretraining} on five downstream tasks \citep{clark2018think, zellers2019hellaswag, sakaguchi2021winogrande, bisk2020piqa}. As shown in \Cref{tab:downstream}, ORCA outperforms Muon on all five tasks. This suggests that the lower pre-training loss of ORCA also leads to better downstream performance.

We also evaluate how the optimization performance translates into token efficiency by measuring the training required to reach a common target loss.
We continued ORCA from its original 51k-step checkpoint, starting the final decay early, and reached a validation loss of 2.318 at approximately 60k steps. The standard Muon run, using its original 100k-step settings, reached the same loss at 100k steps (\Cref{fig:token-efficiency}). Therefore, ORCA used 40\% fewer tokens to reach this target, a 1.66× token-efficiency gain. To save compute, we reused the checkpoint without retuning ORCA for the shorter run: its original 25k-step shaping stage accounts for 41.7\% of the 60k-step budget rather than the tuned default of 25\%.

\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/sec5_lr_sweep.png}
    \captionsetup{skip=2pt}
    \caption{Learning-rate sweep}
    \label{fig:lr-sweep-panel}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/llama350m_validation_loss.png}
    \captionsetup{skip=2pt}
    \caption{LLaMA 350M}
    \label{fig:main-350m}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/llama1b_validation_loss.png}
    \captionsetup{skip=2pt}
    \caption{LLaMA 1.3B}
    \label{fig:main-1b}
  \end{subfigure}
  \captionsetup{skip=2pt}
  \caption{LLaMA pretraining results.}
  \vspace{-8pt}
  \label{fig:lr-sweep}
  \label{fig:main-pretraining}
\end{figure}

\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/llama1b_token_efficiency.png}
    \captionsetup{skip=2pt}
    \caption{Matched-target token efficiency}
    \label{fig:token-efficiency}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/rank_dose_response_scatter.pdf}
    \captionsetup{skip=2pt}
    \caption{Shaping strength $\gamma$}
    \label{fig:rank-dose-response}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/release_fraction_ablation.pdf}
    \captionsetup{skip=2pt}
    \caption{Active-window fraction $\tau$}
    \label{fig:release-point}
  \end{subfigure}
  \captionsetup{skip=2pt}
  \caption{Token efficiency and shaping ablations in LLaMA Pretraining.}
  \vspace{-15pt}
  \label{fig:shaping-strength-timing}
\end{figure}

\begin{table}[t]
  \centering
  \caption{Downstream evaluation on LLaMA 1.3B.}
  \label{tab:downstream}
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{@{}lcccccc@{}}
    \toprule
    Optimizer & ARC-C  & ARC-E & HellaSwag & PIQA & WinoGrande & Avg. \\
    \midrule
    Muon & $0.305\,(0.013)$ & $0.342\,(0.010)$ & $0.549\,(0.005)$
         & $0.705\,(0.011)$ & $0.547\,(0.014)$ & $0.489$ \\
    ORCA & $\mathbf{0.311}\,(0.014)$ & $\mathbf{0.357}\,(0.010)$
         & $\mathbf{0.573}\,(0.005)$ & $\mathbf{0.711}\,(0.011)$
         & $\mathbf{0.553}\,(0.014)$ & $\mathbf{0.501}$ \\
    \bottomrule
  \end{tabular}
  \vspace{-15pt}
  \par\smallskip
\end{table}

\textbf{Qwen3 Pretraining Tasks.} We compare Adam, Muon, and ORCA on Qwen3-style architecture. Within each model scale, all methods share the same common hyperparameters. The Qwen3 0.6B curves cover 50k optimizer steps (about 105B tokens), and the Qwen3 160M curves cover 25k optimizer steps (about 26B tokens).
In both Qwen settings, both sets of loss curves show the same ordering: ORCA may fall temporarily behind Muon early in training, then crosses over and holds the advantage at the
end of the observed interval. The validation-loss improvement of ORCA is therefore not confined to LLaMA, but also reproduces on the Qwen3 architecture.

\textbf{Larger Scale Fine-grained MoE Pretrining.} We observed
router perturbations under a fixed global release point, so we release the
orthogonal constraint layerwise: at $20\%$ of training in the first layer and
at $60\%$ in the last layer, with release times linearly interpolated across
layers. We use top-$4$ routing with $64$ experts in the MoE $0.8$B model
($0.24$B active parameters) and $64$ experts in the MoE $8$B model ($1$B
active parameters) \citep{dai2024deepseekmoe}. Due to computational budget constraints, we focus our comparison on Muon and ORCA. ORCA achieves the lowest final loss at both $25$B and
$50$B tokens for the $0.8$B model, showing that its gain persists as the token
budget increases.
The $8$B experiment extends this result to a larger model trained on $100$B tokens, where ORCA also finishes below Muon (\Cref{fig:moe}). Across these MoE experiments, ORCA reduces final validation loss by $0.020$–$0.025$ relative to Muon.

\textbf{Early orthogonal shaping also benefits other base optimizers.}
We apply the same soft orthogonal shaping step~\eqref{eq:orca-update} to Adam and SOAP on LLaMA 130M \citep{vyas2025soap}. Shaping is active only during the first $25\%$ of training; the base optimizer then continues alone.
For both optimizers, shaping temporarily raises validation loss while active, but the shaped runs overtake their baselines after its removal and finish lower. At 50k steps, it reduces Adam's loss from $2.8824$ to $2.8435$ and SOAP's from $2.8640$ to $2.8271$, gains of $0.0389$ and $0.0369$, respectively. These results show that the benefits of early orthogonal shaping extend beyond Muon to other base optimizers.

\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/qwen3_160m_validation_loss.pdf}
    \captionsetup{skip=2pt}
    \caption{Qwen3 160M}
    \label{fig:qwen-160m}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/qwen3_0p6b_validation_loss.pdf}
    \captionsetup{skip=2pt}
    \caption{Qwen3 0.6B}
    \label{fig:qwen-06b}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/optimizer_generality_validation_loss.pdf}
    \captionsetup{skip=2pt}
    \caption{LLaMA 130M, base optimizers}
    \label{fig:optimizer-generality-panel}
  \end{subfigure}
  \captionsetup{skip=2pt}
  \caption{Validation loss across architectures and base optimizers.}
  \vspace{-15pt}
  \label{fig:qwen}
  \label{fig:optimizer-generality}
\end{figure}

\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/moe_0p8b_0p24b_orca_validation_loss.png}
    \captionsetup{skip=2pt}
    \caption{MoE $0.8$B, $25$B tokens}
    \label{fig:moe-08b-25b}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/moe_0p8b_0p24b_orca_validation_loss_100k.png}
    \captionsetup{skip=2pt}
    \caption{MoE $0.8$B, $50$B tokens}
    \label{fig:moe-08b-50b}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.32\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/moe_8b_1b_orca_validation_loss.png}
    \captionsetup{skip=2pt}
    \caption{MoE $8$B $1$B active, $100$B tokens}
    \label{fig:moe-8b}
  \end{subfigure}
  \captionsetup{skip=2pt}
  \caption{Fine-grained MoE validation loss with layer-wise release.}
  \vspace{-15pt}
  \label{fig:moe}
\end{figure}


==> arxiv/sections/section6.tex <==
\section{Where the Gain Comes From: Controlled Interventions}
\label{sec:interventions}

\Cref{fig:intro-rank-loss} offers an initial view of ORCA's mechanism:
early shaping raises the effective rank, part of this increase persists after
shaping is released, and loss then decreases faster. While
\Cref{sec:main-results} establishes ORCA's optimization gains, in this section
we vary shaping strength and timing, as well as the form of the early spectral
intervention, to isolate their contributions to these gains. Additional
controls for optimizer state and learning-rate schedules are reported
separately in Appendix~\ref{app:controls}.

\textbf{Retained Effective Rank Predicts Post-Release Gain}
We first test whether the effective-rank difference retained after release
tracks ORCA's final gain. Holding all other settings fixed, we sweep the shaping
strength over $\gamma\in\{0,0.05,0.1,0.5,1,2\}$ and measure both the average
post-release effective rank and the final validation loss.
The sweep exhibits a clear dose response. As $\gamma$ increases, the retained
effective rank rises from about $278$ to $335$, while the final validation loss
falls from $2.8466$ to $2.8106$ (\Cref{fig:rank-dose-response}). The relation
flattens at larger $\gamma$, indicating diminishing returns. This
supports retained effective rank as an important variable behind ORCA's
post-release gain.

\noindent\textbf{Release-point sensitivity.}
We first vary the duration of the initial shaping stage over
$\tau\in\{0.10,0.25,0.40,0.55\}$ on LLaMA 130M. Every setting improves over
Muon's final loss of $2.8512$: the four release points reach $2.8210$, $2.8106$,
$2.8107$, and $2.8166$, respectively (\Cref{fig:release-point}). The broad
effective range shows that ORCA does not rely on a precise release point. We use
$\tau=0.25$ by default because it is the shortest tested window in the
best-performing range.

\begin{wrapfigure}[13]{r}{0.38\textwidth}
  \vspace{-\intextsep}
  \centering
  \includegraphics[width=\linewidth]{figures/window_ablation_train_loss.pdf}
  \captionsetup{skip=2pt}
  \caption{Loss curves under different shaping windows on LLaMA 130M.}
  \label{fig:window-ablation}
\end{wrapfigure}

\noindent\textbf{Shaping-window ablation.}
We next compare the default early window $[0,0.25T)$ with middle
$[0.375T,0.625T)$, late $[0.75T,T)$, full-training, and off-then-on
$[0,0.25T)\cup[0.75T,T)$ schedules. Together with the effective-rank dynamics
in \Cref{fig:intro-rank-loss}, \Cref{fig:window-ablation} shows two effects qualitatively consistent with the simplified analysis:
\textbf{(i) shaping is costly while active.} Validation loss rises and remains
on a high plateau whenever shaping is imposed, consistent with persistently
high effective rank restricting the task-adaptive spectrum. \textbf{(ii) The
benefit emerges after release and requires time.} Once shaping is removed, the
retained high-rank state supports faster Muon descent without the same endpoint
restriction. Early shaping leaves the longest released phase and achieves the
lowest final loss. Middle shaping also recovers rapidly and finishes slightly
below Muon, but remains worse than early; late, full, and off-then-on shaping
leave insufficient or no final released phase and fail to recover by the
endpoint. These explain ORCA's two-stage design: raise effective rank
early, then reserve most of training for unconstrained optimization.

\vspace{-4pt}

\subsection{Alternative Early Spectral Interventions}
\label{sec:alternative-interventions}
\vspace{-4pt}
ORCA's mechanistic claim extends beyond soft orthogonal regularization: if raising and retaining effective rank early improves optimization after release, other ways of doing so should yield similar gains. We test this with DiagSVD and Pion-start, comparing them with ORCA and standard Muon in 50k-step LLaMA 130M training. Both alternatives replace soft orthogonal shaping during the first $25\%$ of training; afterward, all variants follow the same Muon dynamics.

DiagSVD directly amplifies updates along weaker singular directions. It
reweights the Muon direction $\widetilde{\mathbf{u}}$ in the basis $\mathbf{U}$ of the left
singular vectors of $\mathbf{W}$:
\begin{equation}
  \widehat{\mathbf{u}}=\mathbf{U}\diag(s_i)\mathbf{U}^\top\widetilde{\mathbf{u}}+s_r(\mathbf{I}-\mathbf{U}\mathbf{U}^\top)\widetilde{\mathbf{u}},
  \qquad
  s_i=1+\theta(i/r)^\delta,
  \label{eq:diagsvd}
\end{equation}
where the singular values are in descending order and $\theta=128$,
$\delta=3$. DiagSVD assigns larger update coefficients to directions associated
with smaller singular values, thereby promoting a
higher effective rank of the weight matrix. The exact and lazy variants refresh
the singular-vector basis every step and every five steps, respectively.
Pion-start instead provides a spectrum-preserving intervention. Given the task
gradient $\mathbf{G}$, it constructs the skew-symmetric generators
\begin{equation}
  \mathbf{G}_{\mathrm{in}}=\mathbf{W}^\top \mathbf{G}-(\mathbf{W}^\top \mathbf{G})^\top,
  \qquad
  \mathbf{G}_{\mathrm{out}}=\mathbf{G}\mathbf{W}^\top-(\mathbf{G}\mathbf{W}^\top)^\top,
  \label{eq:pion-generators}
\end{equation}
and updates the weight from both sides as
\begin{equation}
  \mathbf{W}^+=E_2(\mathbf{A}_{\mathrm{out}})\mathbf{W}E_2(\mathbf{A}_{\mathrm{in}}),
  \qquad
  E_2(\mathbf{A})=\mathbf{I}+\mathbf{A}+\tfrac12\mathbf{A}^2,
  \label{eq:pion-start-update}
\end{equation}
\begin{wrapfigure}{r}{0.40\textwidth}
  \vspace{-\intextsep}
  \centering
  \includegraphics[width=\linewidth]{figures/alternative_rank_shaping_validation_loss.png}
  \captionsetup{skip=2pt}
  \caption{Alternative early spectral interventions on LLaMA 130M,
  released to Muon after $25\%$ of training.}
  \label{fig:alternative-shaping}
\end{wrapfigure}
where $\mathbf{A}_{\mathrm{in}}$ and $\mathbf{A}_{\mathrm{out}}$ are obtained from momentum and
second-moment estimates of the corresponding generators. The underlying
two-sided Lie action preserves the singular spectrum, and hence the effective
rank, during the intervention period; $E_2$ is its second-order approximation.
For Pion-start based methods, whose underlying dynamics preserve the singular spectrum, an orthogonalized start improves the final loss from $2.8505$ with a random start to $2.8371$. This offers an indication that early orthogonality matters. The two DiagSVD variants recover part of ORCA's gain: against Muon's $2.8512$, DiagSVD exact and lazy reach $2.8265$ and $2.8356$, respectively, while ORCA reaches $2.8106$. By amplifying early updates along directions of smaller singular values, DiagSVD improves the final loss even after release. These all indicate early spectral shaping can benefit later optimization.

